DRE: Generating Recommendation Explanations by Aligning Large Language Models at Data-level

Recommendation systems play a crucial role in various domains, suggesting items based on user behavior.However, the lack of transparency in presenting recommendations can lead to user confusion. In this paper, we introduce Data-level Recommendation Explanation (DRE), a non-intrusive explanation framework for black-box recommendation models.Different from existing methods, DRE does not require any intermediary representations of the recommendation model or latent alignment training, mitigating potential performance issues.We propose a data-level alignment method, leveraging large language models to reason relationships between user data and recommended items.Additionally, we address the challenge of enriching the details of the explanation by introducing target-aware user preference distillation, utilizing item reviews. Experimental results on benchmark datasets demonstrate the effectiveness of the DRE in providing accurate and user-centric explanations, enhancing user engagement with recommended item.

==> author.tex <==
\author{Shen Gao}
\authornote{Both authors contributed equally to this research.}
\affiliation{
\institution{University of Electronic Science and Technology of China}
\country{}
% \city{Qingdao}
% \country{China}
}
\email{shengao@pku.edu.cn}

\author{Yifan Wang}
\authornotemark[1]
\affiliation{
\institution{University of Electronic Science and Technology of China}
\country{}
% \city{Qingdao}
% \country{China}
}
\email{yifanwang993w@gmail.com}

\author{Jiabao Fang}
\authornotemark[1]
\affiliation{
\institution{Shandong University}
\country{}
% \city{Qingdao}
% \country{China}
}
\email{jiabaofang@mail.sdu.edu.cn}

\author{Lisi Chen}
\affiliation{
\institution{Renmin University of China}
\country{}
% \city{Beijing}
% \country{China}
}
\email{lchen012@e.ntu.edu.sg}

\author{Peng Han}
\affiliation{
\institution{University of Electronic Science and Technology of China}
\country{}
% \city{Qingdao}
% \country{China}
}
\email{penghan_study@hotmail.com}

\author{Shuo Shang}
\affiliation{
\institution{University of Electronic Science and Technology of China}
\country{}
% \city{Qingdao}
% \country{China}
}
\email{jedi.shang@gmail.com}
